State Estimation in Power Distribution Systems Based on Ensemble Kalman Filtering

State estimation in power distribution systems is a key component for increased reliability and optimal system performance. Well understood in transmission systems, state estimation is now an area of active research in distribution networks. While several snapshot-based approaches have been used to solve this problem, few solutions have been proposed in a dynamic framework. In this paper, a Past-Aware State Estimation (PASE) method is proposed for distribution systems that takes previous estimates into account to improve the accuracy of the current one, using an Ensemble Kalman Filter. Fewer phasor measurements units (PMU) are needed to achieve the same estimation error target than snapshot-based methods. Contrary to current methods, the proposed solution does not embed power flow equations into the estimator. A theoretical formulation is presented to compute a priori the advantages of the proposed method vis-a-vis the state-of-the-art. The proposed approach is validated considering the 33-bus distribution system and using power consumption traces from real households.

==> sections/4-litterature_review.tex <==
%\section{Background and Literature Review}


%\textcolor{red}{[[You should say that nobody has used KF before in DSSE and that the choice of the KF is explained in section X]]} \textcolor{blue}{[[I agreed to this comment during the Skype talk, but after re-reading the paper I realized that we already say this in the introduction. Is it necessary to detail it more here?]]}\textcolor{green}{[[I don't think that this was said: You should say that nobody has used KF before in DSSE}









==> sections/7-load_characterization.tex <==
 \section{Characterization of Load Changes}
        \label{load_model}
        
%The prediction step of the Kalman filter requires a state evolution model which characterizes the state transition and its uncertainty.


%\begin{figure}[t]
%    \centering
%	\includegraphics[width=0.32\textwidth]{figures/laplace_10_houses.eps}
%    \caption{Empirical cumulative distribution function of the load change values and the Laplace fit. The time-step considered is equal to 6 second and 10 houses were aggregated. This illustrates the worst fit over all the fit considered.}
%    \label{fig:cdf_10}
%\end{figure}

==> sections/92-biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
%\vfill
% if you will not have a photo at all:
%\newpage

\begin{IEEEbiographynophoto}{C\^ome Carquex}
is currently working toward the Master's degree in Electrical and Computer Engineering, University of Waterloo, Waterloo, ON, Canada.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Catherine Rosenberg}
(M’89–-SM’96–-F’11) is a Professor, the Canadian Research Chair, and a Fellow of the Canadian Academy of Engineering with the Department of Electrical and Computer Engineering, University of Waterloo, Waterloo, ON, Canada.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Kankar Bhattacharya}
(M'95–-SM'01--F'17) received the Ph.D. degree in electrical engineering from the Indian Institute of Technology, New Delhi, India, in 1993. He was in the faculty of Indira Gandhi Institute of Development Research, Mumbai, India, during 1993–1998, and then the Department of Electric Power Engineering, Chalmers University of Technology, Gothenburg, Sweden, during 1998–2002. He joined the E\&CE Department of the University of Waterloo, Waterloo, ON, Canada, in 2003 where he is currently a full Professor. His research interests are in power system economics and operational aspects.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
